Commissioning of the camera of the first Large Size Telescope of the Cherenkov Telescope Array

The first Large Size Telescope (LST-1) of the Cherenkov Telescope Array has been operational since October 2018 at La Palma, Spain. We report on the results obtained during the camera commissioning. The noise level of the readout is determined as a 0.2 p.e. level. The gain of PMTs are well equalized within 2\% variation, using the calibration flash system. The effect of the night sky background on the signal readout noise as well as the PMT gain estimation are also well evaluated. Trigger thresholds are optimized for the lowest possible gamma-ray energy threshold and the trigger distribution synchronization has been achieved within 1~ns precision. Automatic rate control realizes the stable observation with 1.5\% rate variation over 3 hours. The performance of the novel DAQ system demonstrates a less than 10\% dead time for 15 kHz trigger rate even with sophisticated online data correction.

==> CTA_Acknowledgments_Oct2020.tex <==
%\documentstyle [times,12pt]{article}
%\pagestyle{headings}
%\oddsidemargin=-40pt
%%\evensidemargin=-40pt
%\topmargin=-1cm
%\textwidth=19cm
%\textheight=25.cm 
%\begin{document}  
 
%\pagestyle{empty} 
\begin{center}

{\bf CTA Acknowledgments }

\bigskip\bigskip

We gratefully acknowledge financial support from the following agencies and organizations:

\bigskip

State Committee of Science of Armenia, Armenia;
The Australian Research Council, Astronomy Australia Ltd, The University of Adelaide, Australian National University, Monash University, The University of New South Wales, The University of Sydney, Western Sydney University, Australia;
Federal Ministry of Education, Science and Research, and Innsbruck University, Austria;
Conselho Nacional de Desenvolvimento Cient\'{\i}fico e Tecnol\'{o}gico (CNPq), Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado do Rio de Janeiro (FAPERJ), Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado de S\~{a}o Paulo (FAPESP), Ministry of Science, Technology, Innovations and Communications (MCTIC), Brasil;
Ministry of Education and Science, National RI Roadmap Project DO1-153/28.08.2018, Bulgaria;
The Natural Sciences and Engineering Research Council of Canada and the Canadian Space Agency, Canada;
CONICYT-Chile grants CATA AFB 170002, ANID PIA/APOYO AFB 180002, ACT 1406, FONDECYT-Chile grants, 1161463, 1170171, 1190886, 1171421, 1170345, 1201582, Gemini-ANID 32180007, Chile;
Croatian Science Foundation, Rudjer Boskovic Institute, University of Osijek, University of Rijeka, University of Split, Faculty of Electrical Engineering, Mechanical Engineering and Naval Architecture, University of Zagreb, Faculty of Electrical Engineering and Computing, Croatia;
Ministry of Education, Youth and Sports, MEYS  LM2015046, LM2018105, LTT17006, EU/MEYS CZ.02.1.01/0.0/0.0/16\_013/0001403, CZ.02.1.01/0.0/0.0/18\_046/0016007 and CZ.02.1.01/0.0/0.0/16\_019/0000754, Czech Republic; 
Academy of Finland (grant nr.317636 and 320045), Finland;
Ministry of Higher Education and Research, CNRS-INSU and CNRS-IN2P3, CEA-Irfu, ANR, Regional Council Ile de France, Labex ENIGMASS, OCEVU, OSUG2020 and P2IO, France;
Max Planck Society, BMBF, DESY, Helmholtz Association, Germany;
Department of Atomic Energy, Department of Science and Technology, India;
Istituto Nazionale di Astrofisica (INAF), Istituto Nazionale di Fisica Nucleare (INFN), MIUR, Istituto Nazionale di Astrofisica (INAF-OABRERA) Grant Fondazione Cariplo/Regione Lombardia ID 2014-1980/RST\_ERC, Italy;
ICRR, University of Tokyo, JSPS, MEXT, Japan;
Netherlands Research School for Astronomy (NOVA), Netherlands Organization for Scientific Research (NWO), Netherlands;
University of Oslo, Norway;
Ministry of Science and Higher Education, DIR/WK/2017/12, the National Centre for Research and Development and the National Science Centre, UMO-2016/22/M/ST9/00583, Poland;
Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033, J1-9146, J1-1700, N1-0111, and the Young Researcher program, Slovenia; 
South African Department of Science and Technology and National Research Foundation through the South African Gamma-Ray Astronomy Programme, South Africa;
The Spanish groups acknowledge the Spanish Ministry of Science and Innovation and the Spanish Research State Agency (AEI) through grants AYA2016-79724-C4-1-P, AYA2016-80889-P, AYA2016-76012-C3-1-P, BES-2016-076342, FPA2017-82729-C6-1-R, FPA2017-82729-C6-2-R, FPA2017-82729-C6-3-R, FPA2017-82729-C6-4-R, FPA2017-82729-C6-5-R, FPA2017-82729-C6-6-R, PGC2018-095161-B-I00, PGC2018-095512-B-I00, PID2019-107988GB-C22; the “Centro de Excelencia Severo Ochoa” program through grants no. SEV-2016-0597, SEV-2016-0588, SEV-2017-0709, CEX2019-000920-S; the “Unidad de Excelencia María de Maeztu” program through grant no. MDM-2015-0509; the “Ramón y Cajal” programme through grants RYC-2013-14511, RYC-2017-22665; and the MultiDark Consolider Network FPA2017-90566-REDC. They also acknowledge the Atracci\'on de Talento contract no. 2016-T1/TIC-1542 granted by the Comunidad de Madrid; the “Postdoctoral Junior Leader Fellowship” programme from La Caixa Banking Foundation, grants no.~LCF/BQ/LI18/11630014 and LCF/BQ/PI18/11630012; the “Programa Operativo” FEDER 2014-2020, Consejer\'ia de Econom\'ia y Conocimiento de la Junta de Andaluc\'ia (Ref. 1257737), PAIDI 2020 (Ref. P18-FR-1580) and Universidad de Ja\'en; “Programa Operativo de Crecimiento Inteligente” FEDER 2014-2020 (Ref.~ESFRI-2017-IAC-12), Ministerio de Ciencia e Innovaci\'on, 15\% co-financed by Consejer\'ia de Econom\'ia, Industria, Comercio y Conocimiento del Gobierno de Canarias; the Spanish AEI EQC2018-005094-P FEDER 2014-2020; the European Union’s “Horizon 2020” research and innovation programme under Marie Skłodowska-Curie grant agreement no. 665919; and the ESCAPE project with grant no. GA:824064;
Swedish Research Council, Royal Physiographic Society of Lund, Royal Swedish Academy of Sciences, The Swedish National Infrastructure for Computing (SNIC) at Lunarc (Lund), Sweden;
State Secretariat for Education, Research and Innovation (SERI) and Swiss National Science Foundation (SNSF), Switzerland;
Durham University, Leverhulme Trust, Liverpool University, University of Leicester, University of Oxford, Royal Society, Science and Technology Facilities Council, UK;
U.S. National Science Foundation, U.S. Department of Energy, Argonne National Laboratory, Barnard College, University of California, University of Chicago, Columbia University, Georgia Institute of Technology, Institute for Nuclear and Particle Astrophysics (INPAC-MRPI program), Iowa State University, the Smithsonian Institution, Washington University McDonnell Center for the Space Sciences, The University of Wisconsin and the Wisconsin Alumni Research Foundation, USA.

\bigskip

The research leading to these results has received funding from the European Union's Seventh Framework Programme (FP7/2007-2013) under grant agreements No~262053 and No~317446.
This project is receiving funding from the European Union's Horizon 2020 research and innovation programs under agreement No~676134.
\end{center}
%\end{document}


==> ICRC2021 template/CTA_Acknowledgments_Oct2020.tex <==
%\documentstyle [times,12pt]{article}
%\pagestyle{headings}
%\oddsidemargin=-40pt
%%\evensidemargin=-40pt
%\topmargin=-1cm
%\textwidth=19cm
%\textheight=25.cm 
%\begin{document}  
 
%\pagestyle{empty} 
\begin{center}

{\bf CTA Acknowledgments }

\bigskip\bigskip

We gratefully acknowledge financial support from the following agencies and organizations:

\bigskip

State Committee of Science of Armenia, Armenia;
The Australian Research Council, Astronomy Australia Ltd, The University of Adelaide, Australian National University, Monash University, The University of New South Wales, The University of Sydney, Western Sydney University, Australia;
Federal Ministry of Education, Science and Research, and Innsbruck University, Austria;
Conselho Nacional de Desenvolvimento Cient\'{\i}fico e Tecnol\'{o}gico (CNPq), Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado do Rio de Janeiro (FAPERJ), Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado de S\~{a}o Paulo (FAPESP), Ministry of Science, Technology, Innovations and Communications (MCTIC), Brasil;
Ministry of Education and Science, National RI Roadmap Project DO1-153/28.08.2018, Bulgaria;
The Natural Sciences and Engineering Research Council of Canada and the Canadian Space Agency, Canada;
CONICYT-Chile grants CATA AFB 170002, ANID PIA/APOYO AFB 180002, ACT 1406, FONDECYT-Chile grants, 1161463, 1170171, 1190886, 1171421, 1170345, 1201582, Gemini-ANID 32180007, Chile;
Croatian Science Foundation, Rudjer Boskovic Institute, University of Osijek, University of Rijeka, University of Split, Faculty of Electrical Engineering, Mechanical Engineering and Naval Architecture, University of Zagreb, Faculty of Electrical Engineering and Computing, Croatia;
Ministry of Education, Youth and Sports, MEYS  LM2015046, LM2018105, LTT17006, EU/MEYS CZ.02.1.01/0.0/0.0/16\_013/0001403, CZ.02.1.01/0.0/0.0/18\_046/0016007 and CZ.02.1.01/0.0/0.0/16\_019/0000754, Czech Republic; 
Academy of Finland (grant nr.317636 and 320045), Finland;
Ministry of Higher Education and Research, CNRS-INSU and CNRS-IN2P3, CEA-Irfu, ANR, Regional Council Ile de France, Labex ENIGMASS, OCEVU, OSUG2020 and P2IO, France;
Max Planck Society, BMBF, DESY, Helmholtz Association, Germany;
Department of Atomic Energy, Department of Science and Technology, India;
Istituto Nazionale di Astrofisica (INAF), Istituto Nazionale di Fisica Nucleare (INFN), MIUR, Istituto Nazionale di Astrofisica (INAF-OABRERA) Grant Fondazione Cariplo/Regione Lombardia ID 2014-1980/RST\_ERC, Italy;
ICRR, University of Tokyo, JSPS, MEXT, Japan;
Netherlands Research School for Astronomy (NOVA), Netherlands Organization for Scientific Research (NWO), Netherlands;
University of Oslo, Norway;
Ministry of Science and Higher Education, DIR/WK/2017/12, the National Centre for Research and Development and the National Science Centre, UMO-2016/22/M/ST9/00583, Poland;
Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033, J1-9146, J1-1700, N1-0111, and the Young Researcher program, Slovenia; 
South African Department of Science and Technology and National Research Foundation through the South African Gamma-Ray Astronomy Programme, South Africa;
The Spanish groups acknowledge the Spanish Ministry of Science and Innovation and the Spanish Research State Agency (AEI) through grants AYA2016-79724-C4-1-P, AYA2016-80889-P, AYA2016-76012-C3-1-P, BES-2016-076342, FPA2017-82729-C6-1-R, FPA2017-82729-C6-2-R, FPA2017-82729-C6-3-R, FPA2017-82729-C6-4-R, FPA2017-82729-C6-5-R, FPA2017-82729-C6-6-R, PGC2018-095161-B-I00, PGC2018-095512-B-I00, PID2019-107988GB-C22; the “Centro de Excelencia Severo Ochoa” program through grants no. SEV-2016-0597, SEV-2016-0588, SEV-2017-0709, CEX2019-000920-S; the “Unidad de Excelencia María de Maeztu” program through grant no. MDM-2015-0509; the “Ramón y Cajal” programme through grants RYC-2013-14511, RYC-2017-22665; and the MultiDark Consolider Network FPA2017-90566-REDC. They also acknowledge the Atracci\'on de Talento contract no. 2016-T1/TIC-1542 granted by the Comunidad de Madrid; the “Postdoctoral Junior Leader Fellowship” programme from La Caixa Banking Foundation, grants no.~LCF/BQ/LI18/11630014 and LCF/BQ/PI18/11630012; the “Programa Operativo” FEDER 2014-2020, Consejer\'ia de Econom\'ia y Conocimiento de la Junta de Andaluc\'ia (Ref. 1257737), PAIDI 2020 (Ref. P18-FR-1580) and Universidad de Ja\'en; “Programa Operativo de Crecimiento Inteligente” FEDER 2014-2020 (Ref.~ESFRI-2017-IAC-12), Ministerio de Ciencia e Innovaci\'on, 15\% co-financed by Consejer\'ia de Econom\'ia, Industria, Comercio y Conocimiento del Gobierno de Canarias; the Spanish AEI EQC2018-005094-P FEDER 2014-2020; the European Union’s “Horizon 2020” research and innovation programme under Marie Skłodowska-Curie grant agreement no. 665919; and the ESCAPE project with grant no. GA:824064;
Swedish Research Council, Royal Physiographic Society of Lund, Royal Swedish Academy of Sciences, The Swedish National Infrastructure for Computing (SNIC) at Lunarc (Lund), Sweden;
State Secretariat for Education, Research and Innovation (SERI) and Swiss National Science Foundation (SNSF), Switzerland;
Durham University, Leverhulme Trust, Liverpool University, University of Leicester, University of Oxford, Royal Society, Science and Technology Facilities Council, UK;
U.S. National Science Foundation, U.S. Department of Energy, Argonne National Laboratory, Barnard College, University of California, University of Chicago, Columbia University, Georgia Institute of Technology, Institute for Nuclear and Particle Astrophysics (INPAC-MRPI program), Iowa State University, the Smithsonian Institution, Washington University McDonnell Center for the Space Sciences, The University of Wisconsin and the Wisconsin Alumni Research Foundation, USA.

\bigskip

The research leading to these results has received funding from the European Union's Seventh Framework Programme (FP7/2007-2013) under grant agreements No~262053 and No~317446.
This project is receiving funding from the European Union's Horizon 2020 research and innovation programs under agreement No~676134.
\end{center}
%\end{document}


==> ICRC2021 template/author.tex <==
\scriptsize
\noindent

H. Abe$^{1}$,
A. Aguasca$^{2}$,
I. Agudo$^{3}$,
L. A. Antonelli$^{4}$,
C. Aramo$^{5}$,
T.  Armstrong$^{6}$,
M.  Artero$^{7}$,
K. Asano$^{1}$,
H. Ashkar$^{8}$,
P. Aubert$^{9}$,
A. Baktash$^{10}$,
A. Bamba$^{11}$,
A. Baquero Larriva$^{12}$,
L. Baroncelli$^{13}$,
U. Barres de Almeida$^{14}$,
J. A. Barrio$^{12}$,
I. Batkovic$^{15}$,
J. Becerra González$^{16}$,
M. I. Bernardos$^{15}$,
A. Berti$^{17}$,
N. Biederbeck$^{18}$,
C. Bigongiari$^{4}$,
O. Blanch$^{7}$,
G. Bonnoli$^{3}$,
P. Bordas$^{2}$,
D. Bose$^{19}$,
A. Bulgarelli$^{13}$,
I. Burelli$^{20}$,
M. Buscemi$^{21}$,
M. Cardillo$^{22}$,
S. Caroff$^{9}$,
A. Carosi$^{23}$,
F. Cassol$^{6}$,
M. Cerruti$^{2}$,
Y. Chai$^{17}$,
K. Cheng$^{1}$,
M. Chikawa$^{1}$,
L. Chytka$^{24}$,
J. L. Contreras$^{12}$,
J. Cortina$^{25}$,
H. Costantini$^{6}$,
M. Dalchenko$^{23}$,
A. De Angelis$^{15}$,
M. de Bony de Lavergne$^{9}$,
G. Deleglise$^{9}$,
C. Delgado$^{25}$,
J. Delgado Mengual$^{26}$,
D. della Volpe$^{23}$,
D. Depaoli$^{27,28}$,
F. Di Pierro$^{27}$,
L. Di Venere$^{29}$,
C. Díaz$^{25}$,
R. M. Dominik$^{18}$,
D. Dominis Prester$^{30}$,
A. Donini$^{7}$,
D. Dorner$^{31}$,
M. Doro$^{15}$,
D. Elsässer$^{18}$,
G. Emery$^{23}$,
J. Escudero$^{3}$,
A. Fiasson$^{9}$,
L. Foffano$^{23}$,
M. V. Fonseca$^{12}$,
L. Freixas Coromina$^{25}$,
S. Fukami$^{1}$,
Y. Fukazawa$^{32}$,
E. Garcia$^{9}$,
R. Garcia López$^{16}$,
N. Giglietto$^{33}$,
F. Giordano$^{29}$,
P. Gliwny$^{34}$,
N. Godinovic$^{35}$,
D. Green$^{17}$,
P. Grespan$^{15}$,
S. Gunji$^{36}$,
J. Hackfeld$^{37}$,
D. Hadasch$^{1}$,
A. Hahn$^{17}$,
T.  Hassan$^{25}$,
K. Hayashi$^{38}$,
L. Heckmann$^{17}$,
M. Heller$^{23}$,
J. Herrera Llorente$^{16}$,
K. Hirotani$^{1}$,
D. Hoffmann$^{6}$,
D. Horns$^{10}$,
J. Houles$^{6}$,
M. Hrabovsky$^{24}$,
D. Hrupec$^{39}$,
D. Hui$^{1}$,
M. Hütten$^{17}$,
T. Inada$^{1}$,
Y. Inome$^{1}$,
M. Iori$^{40}$,
K. Ishio$^{34}$,
Y. Iwamura$^{1}$,
M. Jacquemont$^{9}$,
I. Jimenez Martinez$^{25}$,
L. Jouvin$^{7}$,
J. Jurysek$^{41}$,
M. Kagaya$^{1}$,
V. Karas$^{42}$,
H. Katagiri$^{43}$,
J. Kataoka$^{44}$,
D. Kerszberg$^{7}$,
Y. Kobayashi$^{1}$,
A. Kong$^{1}$,
H. Kubo$^{45}$,
J. Kushida$^{46}$,
G. Lamanna$^{9}$,
A. Lamastra$^{4}$,
T. Le Flour$^{9}$,
F. Longo$^{47}$,
R. López-Coto$^{15}$,
M. López-Moya$^{12}$,
A. López-Oramas$^{16}$,
P. L. Luque-Escamilla$^{48}$,
P. Majumdar$^{19,1}$,
M. Makariev$^{49}$,
D. Mandat$^{50}$,
M. Manganaro$^{30}$,
K. Mannheim$^{31}$,
M. Mariotti$^{15}$,
P. Marquez$^{7}$,
G. Marsella$^{21,51}$,
J. Martí$^{48}$,
O. Martinez$^{52}$,
G. Martínez$^{25}$,
M. Martínez$^{7}$,
P. Marusevec$^{53}$,
A. Mas$^{12}$,
G. Maurin$^{9}$,
D. Mazin$^{1,17}$,
E. Mestre Guillen$^{54}$,
S. Micanovic$^{30}$,
D. Miceli$^{9}$,
T. Miener$^{12}$,
J. M. Miranda$^{52}$,
L. D. M. Miranda$^{23}$,
R. Mirzoyan$^{17}$,
T. Mizuno$^{55}$,
E. Molina$^{2}$,
T. Montaruli$^{23}$,
I. Monteiro$^{9}$,
A. Moralejo$^{7}$,
D. Morcuende$^{12}$,
E. Moretti$^{7}$,
A.  Morselli$^{56}$,
K. Mrakovcic$^{30}$,
K. Murase$^{1}$,
A. Nagai$^{23}$,
T. Nakamori$^{36}$,
L. Nickel$^{18}$,
D. Nieto$^{12}$,
M. Nievas$^{16}$,
K. Nishijima$^{46}$,
K. Noda$^{1}$,
D. Nosek$^{57}$,
M. Nöthe$^{18}$,
S. Nozaki$^{45}$,
M. Ohishi$^{1}$,
Y. Ohtani$^{1}$,
T. Oka$^{45}$,
N. Okazaki$^{1}$,
A. Okumura$^{58,59}$,
R. Orito$^{60}$,
J. Otero-Santos$^{16}$,
M. Palatiello$^{20}$,
D. Paneque$^{17}$,
R. Paoletti$^{61}$,
J. M. Paredes$^{2}$,
L. Pavletić$^{30}$,
M. Pech$^{50,62}$,
M. Pecimotika$^{30}$,
V. Poireau$^{9}$,
M. Polo$^{25}$,
E. Prandini$^{15}$,
J. Prast$^{9}$,
C. Priyadarshi$^{7}$,
M. Prouza$^{50}$,
R. Rando$^{15}$,
W. Rhode$^{18}$,
M. Ribó$^{2}$,
V. Rizi$^{63}$,
A.  Rugliancich$^{64}$,
J. E. Ruiz$^{3}$,
T. Saito$^{1}$,
S. Sakurai$^{1}$,
D. A. Sanchez$^{9}$,
T. Šarić$^{35}$,
F. G. Saturni$^{4}$,
J. Scherpenberg$^{17}$,
B. Schleicher$^{31}$,
J. L. Schubert$^{18}$,
F. Schussler$^{8}$,
T. Schweizer$^{17}$,
M. Seglar Arroyo$^{9}$,
R. C. Shellard$^{14}$,
J. Sitarek$^{34}$,
V. Sliusar$^{41}$,
A. Spolon$^{15}$,
J. Strišković$^{39}$,
M. Strzys$^{1}$,
Y. Suda$^{32}$,
Y. Sunada$^{65}$,
H. Tajima$^{58}$,
M. Takahashi$^{1}$,
H. Takahashi$^{32}$,
J. Takata$^{1}$,
R. Takeishi$^{1}$,
P. H. T. Tam$^{1}$,
S. J. Tanaka$^{66}$,
D. Tateishi$^{65}$,
L. A. Tejedor$^{12}$,
P. Temnikov$^{49}$,
Y. Terada$^{65}$,
T. Terzic$^{30}$,
M. Teshima$^{17,1}$,
M. Tluczykont$^{10}$,
F. Tokanai$^{36}$,
D. F. Torres$^{54}$,
P. Travnicek$^{50}$,
S. Truzzi$^{61}$,
M. Vacula$^{24}$,
M. Vázquez Acosta$^{16}$,
V.  Verguilov$^{49}$,
G. Verna$^{6}$,
I. Viale$^{15}$,
C. F. Vigorito$^{27,28}$,
V. Vitale$^{56}$,
I. Vovk$^{1}$,
T. Vuillaume$^{9}$,
R. Walter$^{41}$,
M. Will$^{17}$,
T. Yamamoto$^{67}$,
R. Yamazaki$^{66}$,
T. Yoshida$^{43}$,
T. Yoshikoshi$^{1}$,
and
D. Zarić$^{35}$. \\

\noindent
$^{1}$Institute for Cosmic Ray Research, University of Tokyo.
$^{2}$Departament de Física Quàntica i Astrofísica, Institut de Ciències del Cosmos, Universitat de Barcelona, IEEC-UB.
$^{3}$Instituto de Astrofísica de Andalucía-CSIC.
$^{4}$INAF - Osservatorio Astronomico di Roma.
$^{5}$INFN Sezione di Napoli.
$^{6}$Aix Marseille Univ, CNRS/IN2P3, CPPM.
$^{7}$Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology.
$^{8}$IRFU, CEA, Université Paris-Saclay.
$^{9}$LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS-IN2P3, Annecy.
$^{10}$Universität Hamburg, Institut für Experimentalphysik.
$^{11}$Graduate School of Science, University of Tokyo.
$^{12}$EMFTEL department and IPARCOS, Universidad Complutense de Madrid.
$^{13}$INAF - Osservatorio di Astrofisica e Scienza dello spazio di Bologna.
$^{14}$Centro Brasileiro de Pesquisas Físicas.
$^{15}$INFN Sezione di Padova and Università degli Studi di Padova.
$^{16}$Instituto de Astrofísica de Canarias and Departamento de Astrofísica, Universidad de La Laguna.
$^{17}$Max-Planck-Institut für Physik.
$^{18}$Department of Physics, TU Dortmund University.
$^{19}$Saha Institute of Nuclear Physics.
$^{20}$INFN Sezione di Trieste and Università degli Studi di Udine.
$^{21}$INFN Sezione di Catania.
$^{22}$INAF - Istituto di Astrofisica e Planetologia Spaziali (IAPS).
$^{23}$University of Geneva - Département de physique nucléaire et corpusculaire.
$^{24}$Palacky University Olomouc, Faculty of Science.
$^{25}$CIEMAT.
$^{26}$Port d'Informació Científica.
$^{27}$INFN Sezione di Torino.
$^{28}$Dipartimento di Fisica - Universitá degli Studi di Torino.
$^{29}$INFN Sezione di Bari and Università di Bari.
$^{30}$University of Rijeka, Department of Physics.
$^{31}$Institute for Theoretical Physics and Astrophysics, Universität Würzburg.
$^{32}$Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University.
$^{33}$INFN Sezione di Bari and Politecnico di Bari.
$^{34}$Faculty of Physics and Applied Informatics, University of Lodz.
$^{35}$University of Split, FESB.
$^{36}$Department of Physics, Yamagata University.
$^{37}$Institut für Theoretische Physik, Lehrstuhl IV: Plasma-Astroteilchenphysik, Ruhr-Universität Bochum.
$^{38}$Tohoku University, Astronomical Institute.
$^{39}$Josip Juraj Strossmayer University of Osijek, Department of Physics.
$^{40}$INFN Sezione di Roma La Sapienza.
$^{41}$Department of Astronomy, University of Geneva.
$^{42}$Astronomical Institute of the Czech Academy of Sciences.
$^{43}$Faculty of Science, Ibaraki University.
$^{44}$Faculty of Science and Engineering, Waseda University.
$^{45}$Division of Physics and Astronomy, Graduate School of Science, Kyoto University.
$^{46}$Department of Physics, Tokai University.
$^{47}$INFN Sezione di Trieste and Università degli Studi di Trieste.
$^{48}$Escuela Politécnica Superior de Jaén, Universidad de Jaén.
$^{49}$Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences.
$^{50}$FZU - Institute of Physics of the Czech Academy of Sciences.
$^{51}$Dipartimento di Fisica e Chimica 'E. Segrè' Università degli Studi di Palermo.
$^{52}$Grupo de Electronica, Universidad Complutense de Madrid.
$^{53}$Department of Applied Physics, University of Zagreb.
$^{54}$Institute of Space Sciences (ICE-CSIC), and Institut d'Estudis Espacials de Catalunya (IEEC), and Institució Catalana de Recerca I Estudis Avançats (ICREA).
$^{55}$Hiroshima Astrophysical Science Center, Hiroshima University.
$^{56}$INFN Sezione di Roma Tor Vergata.
$^{57}$Charles University, Institute of Particle and Nuclear Physics.
$^{58}$Institute for Space-Earth Environmental Research, Nagoya University.
$^{59}$Kobayashi-Maskawa Institute (KMI) for the Origin of Particles and the Universe, Nagoya University.
$^{60}$Graduate School of Technology, Industrial and Social Sciences, Tokushima University.
$^{61}$INFN and Università degli Studi di Siena, Dipartimento di Scienze Fisiche, della Terra e dell'Ambiente (DSFTA).
$^{62}$Palacky University Olomouc, Faculty of Science.
$^{63}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{64}$INFN Sezione di Pisa.
$^{65}$Graduate School of Science and Engineering, Saitama University.
$^{66}$Department of Physical Sciences, Aoyama Gakuin University.
$^{67}$Department of Physics, Konan University.


==> author.tex <==
\scriptsize
\noindent

H. Abe$^{1}$,
A. Aguasca$^{2}$,
I. Agudo$^{3}$,
L. A. Antonelli$^{4}$,
C. Aramo$^{5}$,
T.  Armstrong$^{6}$,
M.  Artero$^{7}$,
K. Asano$^{1}$,
H. Ashkar$^{8}$,
P. Aubert$^{9}$,
A. Baktash$^{10}$,
A. Bamba$^{11}$,
A. Baquero Larriva$^{12}$,
L. Baroncelli$^{13}$,
U. Barres de Almeida$^{14}$,
J. A. Barrio$^{12}$,
I. Batkovic$^{15}$,
J. Becerra González$^{16}$,
M. I. Bernardos$^{15}$,
A. Berti$^{17}$,
N. Biederbeck$^{18}$,
C. Bigongiari$^{4}$,
O. Blanch$^{7}$,
G. Bonnoli$^{3}$,
P. Bordas$^{2}$,
D. Bose$^{19}$,
A. Bulgarelli$^{13}$,
I. Burelli$^{20}$,
M. Buscemi$^{21}$,
M. Cardillo$^{22}$,
S. Caroff$^{9}$,
A. Carosi$^{23}$,
F. Cassol$^{6}$,
M. Cerruti$^{2}$,
Y. Chai$^{17}$,
K. Cheng$^{1}$,
M. Chikawa$^{1}$,
L. Chytka$^{24}$,
J. L. Contreras$^{12}$,
J. Cortina$^{25}$,
H. Costantini$^{6}$,
M. Dalchenko$^{23}$,
A. De Angelis$^{15}$,
M. de Bony de Lavergne$^{9}$,
G. Deleglise$^{9}$,
C. Delgado$^{25}$,
J. Delgado Mengual$^{26}$,
D. della Volpe$^{23}$,
D. Depaoli$^{27,28}$,
F. Di Pierro$^{27}$,
L. Di Venere$^{29}$,
C. Díaz$^{25}$,
R. M. Dominik$^{18}$,
D. Dominis Prester$^{30}$,
A. Donini$^{7}$,
D. Dorner$^{31}$,
M. Doro$^{15}$,
D. Elsässer$^{18}$,
G. Emery$^{23}$,
J. Escudero$^{3}$,
A. Fiasson$^{9}$,
L. Foffano$^{23}$,
M. V. Fonseca$^{12}$,
L. Freixas Coromina$^{25}$,
S. Fukami$^{1}$,
Y. Fukazawa$^{32}$,
E. Garcia$^{9}$,
R. Garcia López$^{16}$,
N. Giglietto$^{33}$,
F. Giordano$^{29}$,
P. Gliwny$^{34}$,
N. Godinovic$^{35}$,
D. Green$^{17}$,
P. Grespan$^{15}$,
S. Gunji$^{36}$,
J. Hackfeld$^{37}$,
D. Hadasch$^{1}$,
A. Hahn$^{17}$,
T.  Hassan$^{25}$,
K. Hayashi$^{38}$,
L. Heckmann$^{17}$,
M. Heller$^{23}$,
J. Herrera Llorente$^{16}$,
K. Hirotani$^{1}$,
D. Hoffmann$^{6}$,
D. Horns$^{10}$,
J. Houles$^{6}$,
M. Hrabovsky$^{24}$,
D. Hrupec$^{39}$,
D. Hui$^{1}$,
M. Hütten$^{17}$,
T. Inada$^{1}$,
Y. Inome$^{1}$,
M. Iori$^{40}$,
K. Ishio$^{34}$,
Y. Iwamura$^{1}$,
M. Jacquemont$^{9}$,
I. Jimenez Martinez$^{25}$,
L. Jouvin$^{7}$,
J. Jurysek$^{41}$,
M. Kagaya$^{1}$,
V. Karas$^{42}$,
H. Katagiri$^{43}$,
J. Kataoka$^{44}$,
D. Kerszberg$^{7}$,
Y. Kobayashi$^{1}$,
A. Kong$^{1}$,
H. Kubo$^{45}$,
J. Kushida$^{46}$,
G. Lamanna$^{9}$,
A. Lamastra$^{4}$,
T. Le Flour$^{9}$,
F. Longo$^{47}$,
R. López-Coto$^{15}$,
M. López-Moya$^{12}$,
A. López-Oramas$^{16}$,
P. L. Luque-Escamilla$^{48}$,
P. Majumdar$^{19,1}$,
M. Makariev$^{49}$,
D. Mandat$^{50}$,
M. Manganaro$^{30}$,
K. Mannheim$^{31}$,
M. Mariotti$^{15}$,
P. Marquez$^{7}$,
G. Marsella$^{21,51}$,
J. Martí$^{48}$,
O. Martinez$^{52}$,
G. Martínez$^{25}$,
M. Martínez$^{7}$,
P. Marusevec$^{53}$,
A. Mas$^{12}$,
G. Maurin$^{9}$,
D. Mazin$^{1,17}$,
E. Mestre Guillen$^{54}$,
S. Micanovic$^{30}$,
D. Miceli$^{9}$,
T. Miener$^{12}$,
J. M. Miranda$^{52}$,
L. D. M. Miranda$^{23}$,
R. Mirzoyan$^{17}$,
T. Mizuno$^{55}$,
E. Molina$^{2}$,
T. Montaruli$^{23}$,
I. Monteiro$^{9}$,
A. Moralejo$^{7}$,
D. Morcuende$^{12}$,
E. Moretti$^{7}$,
A.  Morselli$^{56}$,
K. Mrakovcic$^{30}$,
K. Murase$^{1}$,
A. Nagai$^{23}$,
T. Nakamori$^{36}$,
L. Nickel$^{18}$,
D. Nieto$^{12}$,
M. Nievas$^{16}$,
K. Nishijima$^{46}$,
K. Noda$^{1}$,
D. Nosek$^{57}$,
M. Nöthe$^{18}$,
S. Nozaki$^{45}$,
M. Ohishi$^{1}$,
Y. Ohtani$^{1}$,
T. Oka$^{45}$,
N. Okazaki$^{1}$,
A. Okumura$^{58,59}$,
R. Orito$^{60}$,
J. Otero-Santos$^{16}$,
M. Palatiello$^{20}$,
D. Paneque$^{17}$,
R. Paoletti$^{61}$,
J. M. Paredes$^{2}$,
L. Pavletić$^{30}$,
M. Pech$^{50,62}$,
M. Pecimotika$^{30}$,
V. Poireau$^{9}$,
M. Polo$^{25}$,
E. Prandini$^{15}$,
J. Prast$^{9}$,
C. Priyadarshi$^{7}$,
M. Prouza$^{50}$,
R. Rando$^{15}$,
W. Rhode$^{18}$,
M. Ribó$^{2}$,
V. Rizi$^{63}$,
A.  Rugliancich$^{64}$,
J. E. Ruiz$^{3}$,
T. Saito$^{1}$,
S. Sakurai$^{1}$,
D. A. Sanchez$^{9}$,
T. Šarić$^{35}$,
F. G. Saturni$^{4}$,
J. Scherpenberg$^{17}$,
B. Schleicher$^{31}$,
J. L. Schubert$^{18}$,
F. Schussler$^{8}$,
T. Schweizer$^{17}$,
M. Seglar Arroyo$^{9}$,
R. C. Shellard$^{14}$,
J. Sitarek$^{34}$,
V. Sliusar$^{41}$,
A. Spolon$^{15}$,
J. Strišković$^{39}$,
M. Strzys$^{1}$,
Y. Suda$^{32}$,
Y. Sunada$^{65}$,
H. Tajima$^{58}$,
M. Takahashi$^{1}$,
H. Takahashi$^{32}$,
J. Takata$^{1}$,
R. Takeishi$^{1}$,
P. H. T. Tam$^{1}$,
S. J. Tanaka$^{66}$,
D. Tateishi$^{65}$,
L. A. Tejedor$^{12}$,
P. Temnikov$^{49}$,
Y. Terada$^{65}$,
T. Terzic$^{30}$,
M. Teshima$^{17,1}$,
M. Tluczykont$^{10}$,
F. Tokanai$^{36}$,
D. F. Torres$^{54}$,
P. Travnicek$^{50}$,
S. Truzzi$^{61}$,
M. Vacula$^{24}$,
M. Vázquez Acosta$^{16}$,
V.  Verguilov$^{49}$,
G. Verna$^{6}$,
I. Viale$^{15}$,
C. F. Vigorito$^{27,28}$,
V. Vitale$^{56}$,
I. Vovk$^{1}$,
T. Vuillaume$^{9}$,
R. Walter$^{41}$,
M. Will$^{17}$,
T. Yamamoto$^{67}$,
R. Yamazaki$^{66}$,
T. Yoshida$^{43}$,
T. Yoshikoshi$^{1}$,
and
D. Zarić$^{35}$. \\

\noindent
$^{1}$Institute for Cosmic Ray Research, University of Tokyo.
$^{2}$Departament de Física Quàntica i Astrofísica, Institut de Ciències del Cosmos, Universitat de Barcelona, IEEC-UB.
$^{3}$Instituto de Astrofísica de Andalucía-CSIC.
$^{4}$INAF - Osservatorio Astronomico di Roma.
$^{5}$INFN Sezione di Napoli.
$^{6}$Aix Marseille Univ, CNRS/IN2P3, CPPM.
$^{7}$Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology.
$^{8}$IRFU, CEA, Université Paris-Saclay.
$^{9}$LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS-IN2P3, Annecy.
$^{10}$Universität Hamburg, Institut für Experimentalphysik.
$^{11}$Graduate School of Science, University of Tokyo.
$^{12}$EMFTEL department and IPARCOS, Universidad Complutense de Madrid.
$^{13}$INAF - Osservatorio di Astrofisica e Scienza dello spazio di Bologna.
$^{14}$Centro Brasileiro de Pesquisas Físicas.
$^{15}$INFN Sezione di Padova and Università degli Studi di Padova.
$^{16}$Instituto de Astrofísica de Canarias and Departamento de Astrofísica, Universidad de La Laguna.
$^{17}$Max-Planck-Institut für Physik.
$^{18}$Department of Physics, TU Dortmund University.
$^{19}$Saha Institute of Nuclear Physics.
$^{20}$INFN Sezione di Trieste and Università degli Studi di Udine.
$^{21}$INFN Sezione di Catania.
$^{22}$INAF - Istituto di Astrofisica e Planetologia Spaziali (IAPS).
$^{23}$University of Geneva - Département de physique nucléaire et corpusculaire.
$^{24}$Palacky University Olomouc, Faculty of Science.
$^{25}$CIEMAT.
$^{26}$Port d'Informació Científica.
$^{27}$INFN Sezione di Torino.
$^{28}$Dipartimento di Fisica - Universitá degli Studi di Torino.
$^{29}$INFN Sezione di Bari and Università di Bari.
$^{30}$University of Rijeka, Department of Physics.
$^{31}$Institute for Theoretical Physics and Astrophysics, Universität Würzburg.
$^{32}$Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University.
$^{33}$INFN Sezione di Bari and Politecnico di Bari.
$^{34}$Faculty of Physics and Applied Informatics, University of Lodz.
$^{35}$University of Split, FESB.
$^{36}$Department of Physics, Yamagata University.
$^{37}$Institut für Theoretische Physik, Lehrstuhl IV: Plasma-Astroteilchenphysik, Ruhr-Universität Bochum.
$^{38}$Tohoku University, Astronomical Institute.
$^{39}$Josip Juraj Strossmayer University of Osijek, Department of Physics.
$^{40}$INFN Sezione di Roma La Sapienza.
$^{41}$Department of Astronomy, University of Geneva.
$^{42}$Astronomical Institute of the Czech Academy of Sciences.
$^{43}$Faculty of Science, Ibaraki University.
$^{44}$Faculty of Science and Engineering, Waseda University.
$^{45}$Division of Physics and Astronomy, Graduate School of Science, Kyoto University.
$^{46}$Department of Physics, Tokai University.
$^{47}$INFN Sezione di Trieste and Università degli Studi di Trieste.
$^{48}$Escuela Politécnica Superior de Jaén, Universidad de Jaén.
$^{49}$Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences.
$^{50}$FZU - Institute of Physics of the Czech Academy of Sciences.
$^{51}$Dipartimento di Fisica e Chimica 'E. Segrè' Università degli Studi di Palermo.
$^{52}$Grupo de Electronica, Universidad Complutense de Madrid.
$^{53}$Department of Applied Physics, University of Zagreb.
$^{54}$Institute of Space Sciences (ICE-CSIC), and Institut d'Estudis Espacials de Catalunya (IEEC), and Institució Catalana de Recerca I Estudis Avançats (ICREA).
$^{55}$Hiroshima Astrophysical Science Center, Hiroshima University.
$^{56}$INFN Sezione di Roma Tor Vergata.
$^{57}$Charles University, Institute of Particle and Nuclear Physics.
$^{58}$Institute for Space-Earth Environmental Research, Nagoya University.
$^{59}$Kobayashi-Maskawa Institute (KMI) for the Origin of Particles and the Universe, Nagoya University.
$^{60}$Graduate School of Technology, Industrial and Social Sciences, Tokushima University.
$^{61}$INFN and Università degli Studi di Siena, Dipartimento di Scienze Fisiche, della Terra e dell'Ambiente (DSFTA).
$^{62}$Palacky University Olomouc, Faculty of Science.
$^{63}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{64}$INFN Sezione di Pisa.
$^{65}$Graduate School of Science and Engineering, Saitama University.
$^{66}$Department of Physical Sciences, Aoyama Gakuin University.
$^{67}$Department of Physics, Konan University.


==> authorDM.tex <==
\scriptsize
\noindent
H. Abe$^{1}$,
A. Aguasca$^{2}$,
I. Agudo$^{3}$,
L. A. Antonelli$^{4}$,
C. Aramo$^{5}$,
T.  Armstrong$^{6}$,
M.  Artero$^{7}$,
K. Asano$^{1}$,
H. Ashkar$^{8}$,
P. Aubert$^{9}$,
A. Baktash$^{10}$,
A. Bamba$^{11}$,
A. Baquero Larriva$^{12}$,
L. Baroncelli$^{13}$,
U. Barres de Almeida$^{14}$,
J. A. Barrio$^{12}$,
I. Batkovic$^{15}$,
J. Becerra González$^{16}$,
M. I. Bernardos$^{15}$,
A. Berti$^{17}$,
N. Biederbeck$^{18}$,
C. Bigongiari$^{4}$,
O. Blanch$^{7}$,
G. Bonnoli$^{3}$,
P. Bordas$^{2}$,
D. Bose$^{19}$,
A. Bulgarelli$^{13}$,
I. Burelli$^{20}$,
M. Buscemi$^{21}$,
M. Cardillo$^{22}$,
S. Caroff$^{9}$,
A. Carosi$^{23}$,
F. Cassol$^{6}$,
M. Cerruti$^{2}$,
Y. Chai$^{17}$,
K. Cheng$^{1}$,
M. Chikawa$^{1}$,
L. Chytka$^{24}$,
J. L. Contreras$^{12}$,
J. Cortina$^{25}$,
H. Costantini$^{6}$,
M. Dalchenko$^{23}$,
A. De Angelis$^{15}$,
M. de Bony de Lavergne$^{9}$,
G. Deleglise$^{9}$,
C. Delgado$^{25}$,
J. Delgado Mengual$^{26}$,
D. della Volpe$^{23}$,
D. Depaoli$^{27,28}$,
F. Di Pierro$^{27}$,
L. Di Venere$^{29}$,
C. Díaz$^{25}$,
R. M. Dominik$^{18}$,
D. Dominis Prester$^{30}$,
A. Donini$^{7}$,
D. Dorner$^{31}$,
M. Doro$^{15}$,
D. Elsässer$^{18}$,
G. Emery$^{23}$,
J. Escudero$^{3}$,
A. Fiasson$^{9}$,
L. Foffano$^{23}$,
M. V. Fonseca$^{12}$,
L. Freixas Coromina$^{25}$,
S. Fukami$^{1}$,
Y. Fukazawa$^{32}$,
E. Garcia$^{9}$,
R. Garcia López$^{16}$,
N. Giglietto$^{33}$,
F. Giordano$^{29}$,
P. Gliwny$^{34}$,
N. Godinovic$^{35}$,
D. Green$^{17}$,
P. Grespan$^{15}$,
S. Gunji$^{36}$,
J. Hackfeld$^{37}$,
D. Hadasch$^{1}$,
A. Hahn$^{17}$,
T.  Hassan$^{25}$,
K. Hayashi$^{38}$,
L. Heckmann$^{17}$,
M. Heller$^{23}$,
J. Herrera Llorente$^{16}$,
K. Hirotani$^{1}$,
D. Hoffmann$^{6}$,
D. Horns$^{10}$,
J. Houles$^{6}$,
M. Hrabovsky$^{24}$,
D. Hrupec$^{39}$,
D. Hui$^{1}$,
M. Hütten$^{17}$,
T. Inada$^{1}$,
Y. Inome$^{1}$,
M. Iori$^{40}$,
K. Ishio$^{34}$,
Y. Iwamura$^{1}$,
M. Jacquemont$^{9}$,
I. Jimenez Martinez$^{25}$,
L. Jouvin$^{7}$,
J. Jurysek$^{41}$,
M. Kagaya$^{1}$,
V. Karas$^{42}$,
H. Katagiri$^{43}$,
J. Kataoka$^{44}$,
D. Kerszberg$^{7}$,
Y. Kobayashi$^{1}$,
A. Kong$^{1}$,
H. Kubo$^{45}$,
J. Kushida$^{46}$,
G. Lamanna$^{9}$,
A. Lamastra$^{4}$,
T. Le Flour$^{9}$,
F. Longo$^{47}$,
R. López-Coto$^{15}$,
M. López-Moya$^{12}$,
A. López-Oramas$^{16}$,
P. L. Luque-Escamilla$^{48}$,
P. Majumdar$^{19,1}$,
M. Makariev$^{49}$,
D. Mandat$^{50}$,
M. Manganaro$^{30}$,
K. Mannheim$^{31}$,
M. Mariotti$^{15}$,
P. Marquez$^{7}$,
G. Marsella$^{21,51}$,
J. Martí$^{48}$,
O. Martinez$^{52}$,
G. Martínez$^{25}$,
M. Martínez$^{7}$,
P. Marusevec$^{53}$,
A. Mas$^{12}$,
G. Maurin$^{9}$,
D. Mazin$^{1,17}$,
E. Mestre Guillen$^{54}$,
S. Micanovic$^{30}$,
D. Miceli$^{9}$,
T. Miener$^{12}$,
J. M. Miranda$^{52}$,
L. D. M. Miranda$^{23}$,
R. Mirzoyan$^{17}$,
T. Mizuno$^{55}$,
E. Molina$^{2}$,
T. Montaruli$^{23}$,
I. Monteiro$^{9}$,
A. Moralejo$^{7}$,
D. Morcuende$^{12}$,
E. Moretti$^{7}$,
A.  Morselli$^{56}$,
K. Mrakovcic$^{30}$,
K. Murase$^{1}$,
A. Nagai$^{23}$,
T. Nakamori$^{36}$,
L. Nickel$^{18}$,
D. Nieto$^{12}$,
M. Nievas$^{16}$,
K. Nishijima$^{46}$,
K. Noda$^{1}$,
D. Nosek$^{57}$,
M. Nöthe$^{18}$,
S. Nozaki$^{45}$,
M. Ohishi$^{1}$,
Y. Ohtani$^{1}$,
T. Oka$^{45}$,
N. Okazaki$^{1}$,
A. Okumura$^{58,59}$,
R. Orito$^{60}$,
J. Otero-Santos$^{16}$,
M. Palatiello$^{20}$,
D. Paneque$^{17}$,
R. Paoletti$^{61}$,
J. M. Paredes$^{2}$,
L. Pavletić$^{30}$,
M. Pech$^{50,62}$,
M. Pecimotika$^{30}$,
V. Poireau$^{9}$,
M. Polo$^{25}$,
E. Prandini$^{15}$,
J. Prast$^{9}$,
C. Priyadarshi$^{7}$,
M. Prouza$^{50}$,
R. Rando$^{15}$,
W. Rhode$^{18}$,
M. Ribó$^{2}$,
V. Rizi$^{63}$,
A.  Rugliancich$^{64}$,
J. E. Ruiz$^{3}$,
T. Saito$^{1}$,
S. Sakurai$^{1}$,
D. A. Sanchez$^{9}$,
T. Šarić$^{35}$,
F. G. Saturni$^{4}$,
J. Scherpenberg$^{17}$,
B. Schleicher$^{31}$,
J. L. Schubert$^{18}$,
F. Schussler$^{8}$,
T. Schweizer$^{17}$,
M. Seglar Arroyo$^{9}$,
R. C. Shellard$^{14}$,
J. Sitarek$^{34}$,
V. Sliusar$^{41}$,
A. Spolon$^{15}$,
J. Strišković$^{39}$,
M. Strzys$^{1}$,
Y. Suda$^{32}$,
Y. Sunada$^{65}$,
H. Tajima$^{58}$,
M. Takahashi$^{1}$,
H. Takahashi$^{32}$,
J. Takata$^{1}$,
R. Takeishi$^{1}$,
P. H. T. Tam$^{1}$,
S. J. Tanaka$^{66}$,
D. Tateishi$^{65}$,
L. A. Tejedor$^{12}$,
P. Temnikov$^{49}$,
Y. Terada$^{65}$,
T. Terzic$^{30}$,
M. Teshima$^{17,1}$,
M. Tluczykont$^{10}$,
F. Tokanai$^{36}$,
D. F. Torres$^{54}$,
P. Travnicek$^{50}$,
S. Truzzi$^{61}$,
M. Vacula$^{24}$,
M. Vázquez Acosta$^{16}$,
V.  Verguilov$^{49}$,
G. Verna$^{6}$,
I. Viale$^{15}$,
C. F. Vigorito$^{27,28}$,
V. Vitale$^{56}$,
I. Vovk$^{1}$,
T. Vuillaume$^{9}$,
R. Walter$^{41}$,
M. Will$^{17}$,
T. Yamamoto$^{67}$,
R. Yamazaki$^{66}$,
T. Yoshida$^{43}$,
T. Yoshikoshi$^{1}$,
and
D. Zarić$^{35}$. \\

\noindent
$^{1}$Institute for Cosmic Ray Research, University of Tokyo.
$^{2}$Departament de Física Quàntica i Astrofísica, Institut de Ciències del Cosmos, Universitat de Barcelona, IEEC-UB.
$^{3}$Instituto de Astrofísica de Andalucía-CSIC.
$^{4}$INAF - Osservatorio Astronomico di Roma.
$^{5}$INFN Sezione di Napoli.
$^{6}$Aix Marseille Univ, CNRS/IN2P3, CPPM.
$^{7}$Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology.
$^{8}$IRFU, CEA, Université Paris-Saclay.
$^{9}$LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS-IN2P3, Annecy.
$^{10}$Universität Hamburg, Institut für Experimentalphysik.
$^{11}$Graduate School of Science, University of Tokyo.
$^{12}$EMFTEL department and IPARCOS, Universidad Complutense de Madrid.
$^{13}$INAF - Osservatorio di Astrofisica e Scienza dello spazio di Bologna.
$^{14}$Centro Brasileiro de Pesquisas Físicas.
$^{15}$INFN Sezione di Padova and Università degli Studi di Padova.
$^{16}$Instituto de Astrofísica de Canarias and Departamento de Astrofísica, Universidad de La Laguna.
$^{17}$Max-Planck-Institut für Physik.
$^{18}$Department of Physics, TU Dortmund University.
$^{19}$Saha Institute of Nuclear Physics.
$^{20}$INFN Sezione di Trieste and Università degli Studi di Udine.
$^{21}$INFN Sezione di Catania.
$^{22}$INAF - Istituto di Astrofisica e Planetologia Spaziali (IAPS).
$^{23}$University of Geneva - Département de physique nucléaire et corpusculaire.
$^{24}$Palacky University Olomouc, Faculty of Science.
$^{25}$CIEMAT.
$^{26}$Port d'Informació Científica.
$^{27}$INFN Sezione di Torino.
$^{28}$Dipartimento di Fisica - Universitá degli Studi di Torino.
$^{29}$INFN Sezione di Bari and Università di Bari.
$^{30}$University of Rijeka, Department of Physics.
$^{31}$Institute for Theoretical Physics and Astrophysics, Universität Würzburg.
$^{32}$Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University.
$^{33}$INFN Sezione di Bari and Politecnico di Bari.
$^{34}$Faculty of Physics and Applied Informatics, University of Lodz.
$^{35}$University of Split, FESB.
$^{36}$Department of Physics, Yamagata University.
$^{37}$Institut für Theoretische Physik, Lehrstuhl IV: Plasma-Astroteilchenphysik, Ruhr-Universität Bochum.
$^{38}$Tohoku University, Astronomical Institute.
$^{39}$Josip Juraj Strossmayer University of Osijek, Department of Physics.
$^{40}$INFN Sezione di Roma La Sapienza.
$^{41}$Department of Astronomy, University of Geneva.
$^{42}$Astronomical Institute of the Czech Academy of Sciences.
$^{43}$Faculty of Science, Ibaraki University.
$^{44}$Faculty of Science and Engineering, Waseda University.
$^{45}$Division of Physics and Astronomy, Graduate School of Science, Kyoto University.
$^{46}$Department of Physics, Tokai University.
$^{47}$INFN Sezione di Trieste and Università degli Studi di Trieste.
$^{48}$Escuela Politécnica Superior de Jaén, Universidad de Jaén.
$^{49}$Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences.
$^{50}$FZU - Institute of Physics of the Czech Academy of Sciences.
$^{51}$Dipartimento di Fisica e Chimica 'E. Segrè' Università degli Studi di Palermo.
$^{52}$Grupo de Electronica, Universidad Complutense de Madrid.
$^{53}$Department of Applied Physics, University of Zagreb.
$^{54}$Institute of Space Sciences (ICE-CSIC), and Institut d'Estudis Espacials de Catalunya (IEEC), and Institució Catalana de Recerca I Estudis Avançats (ICREA).
$^{55}$Hiroshima Astrophysical Science Center, Hiroshima University.
$^{56}$INFN Sezione di Roma Tor Vergata.
$^{57}$Charles University, Institute of Particle and Nuclear Physics.
$^{58}$Institute for Space-Earth Environmental Research, Nagoya University.
$^{59}$Kobayashi-Maskawa Institute (KMI) for the Origin of Particles and the Universe, Nagoya University.
$^{60}$Graduate School of Technology, Industrial and Social Sciences, Tokushima University.
$^{61}$INFN and Università degli Studi di Siena, Dipartimento di Scienze Fisiche, della Terra e dell'Ambiente (DSFTA).
$^{62}$Palacky University Olomouc, Faculty of Science.
$^{63}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{64}$INFN Sezione di Pisa.
$^{65}$Graduate School of Science and Engineering, Saitama University.
$^{66}$Department of Physical Sciences, Aoyama Gakuin University.
$^{67}$Department of Physics, Konan University.

